Feasibility-Guided Safety-Aware Model Predictive Control for Jump Markov Linear Systems

In this paper, we present a controller framework that synthesizes control policies for Jump Markov Linear Systems subject to stochastic mode switches and imperfect mode estimation. Our approach builds on safe and robust methods for Model Predictive Control (MPC), but in contrast to existing approaches that either optimize without regard to feasibility or utilize soft constraints that increase computational requirements, we employ a safe and robust control approach informed by the feasibility of the optimization problem. We formulate and encode finite horizon safety for multiple model systems in our MPC design using Control Barrier Functions (CBFs). When subject to inaccurate hybrid state estimation, our feasibility-guided MPC generates a control policy that is maximally robust to uncertainty in the system's modes. We evaluate our approach on an orbital rendezvous problem and a six degree-of-freedom hexacopter under several scenarios and benchmarks to demonstrate the utility of the framework. Results indicate that the proposed technique of maximizing the robustness horizon, and the use of CBFs for safety awareness, improve the overall safety and performance of MPC for Jump Markov Linear Systems.

==> IROS2024/Bin/Notes.tex <==
Read papers:

% http://larsblackmore.com/BlackmoreTAC08.pdf
% http://ames.caltech.edu/molnar2021model.pdf
% https://ieeexplore.ieee.org/abstract/document/9304395
% https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9682854
% https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9691815
% https://arxiv.org/pdf/2007.11718.pdf
% https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=7040372


Barrier notes:

https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=9303896

https://reader.elsevier.com/reader/sd/pii/S0005109822005489?token=A923160186DD009D8146704FD804CBEC72FD45B3C73D5FFF43B5707FFA7CC9E4D79566763E8AAD1E8DE0C473DC9B133A&originRegion=us-east-1&originCreation=20230325034722

https://arxiv.org/pdf/2104.00101.pdf

https://arxiv.org/pdf/1903.11199.pdf

\begin{definition}[Control Barrier Function, \cite{ames2016control}]
\RM{Re-word this} The existence of a CBF implies that there is a controller of deterministic nature for which the set C is forward invariant given the system. Given a function $h$, the function $B$ is a CBF if there exits locally Lipschitz class $\mathcal{K}$ functions $\alpha_{1}, \alpha_{2}$, such that:
\begin{align}
\label{condition}
\begin{split}
    & \frac{1}{\alpha_{1}(h(x))} \leq B(x) \leq \frac{1}{\alpha_{2}(h(x))} \\
    & \inf_{u\in U} 
    \left [ 
    L_{f}B(x) + L_{g}B(x)u - \frac{\gamma}{B(x)}
    \right] \leq 0
\end{split}
\end{align}
\RM{Rayan: check the last part of this function, it is specific for some barrier shape.}
in which $L_{p}q(x):= \bigtriangledown q(x)\cdot p(x)$ is a Lie derivative operator. 
\end{definition}


% \begin{figure}
%     \centering
%     \subfigure[]{\includegraphics[width=0.24\textwidth]{}} 
%     \subfigure[]{\includegraphics[width=0.24\textwidth]{}}
%     \subfigure[]{\includegraphics[width=0.24\textwidth]{}}
%     \caption{(a) blah (b) blah (c) blah (d) blah}
%     \label{fig:foobar}
% \end{figure}


% \begin{figure}[b!]
%   \centering
%     \includegraphics[width=4in]{CDC2023/Figures/comparelowtol.pdf}
%     \caption{}
%     \label{fig:twomode}
% \end{figure}
% \begin{figure}[b!]
%   \centering
%     \includegraphics[width=4in]{CDC2023/Figures/comparelowtol7.pdf}
%     \caption{Seven Mode Planner Comparison. State trajectories for the non-robust, unitary-consensus, and max-consensus approaches subject to a rotor failure induced at time $t=1s$ and a delayed IMM diagnosis of $+0.15s$.}
%     \label{fig:sevenmode}
% \end{figure}
% \begin{figure}[b!]
%   \centering
%     \includegraphics[width=4in]{CDC2023/Figures/legend.png}
%     \caption{}
%     \label{fig:legend}
% \end{figure}
% \begin{figure}[b!]
% \centering
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=1.0\linewidth]{CDC2023/Figures/3dtrajectory.png}
%   \caption{Visualization of the trajectories in 3D-space.}
%   \label{fig:sub1}
% \end{subfigure}%
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=0.9\linewidth]{CDC2023/Figures/topview.png}
%   \caption{Top-view of the trajectories.}
%   \label{fig:sub2}
% \end{subfigure}
% \caption{Trajectory of the three methods: (1) non-robust, (2) unitary-consensus, and (3) maximum-consensus. It is observed that the maximum consensus algorithm is the only method capable of safely guiding the hexacopter to the goal state, even under a stochastic rotor failure.}
% \label{fig:trajectory}
% \end{figure}


% \begin{figure*}[t!]
% \label{fullcomp}
% \centering
% \begin{subfigure}{.40\textwidth}
%   \centering
%   \vspace{-5mm}
%   \includegraphics[width=1.0\textwidth]{CDC2023/Figures/comparelowtol.pdf}
%   \caption{Two Mode Planner Comparison. }
%   \label{fig:submodes1}
% \end{subfigure}%
% \begin{subfigure}{.19\textwidth}
%   \centering
%    \begin{minipage}{5cm}
%    \vspace{-10cm} 
%   \hspace{5mm}\includegraphics[width=0.5\textwidth]{CDC2023/Figures/legend.png}
%     \end{minipage}
%   \label{fig:submodes2}
% \end{subfigure}
% \begin{subfigure}{0.40\textwidth}
%   \centering
%   \includegraphics[width=1.0\textwidth]{CDC2023/Figures/comparelowtol7.pdf}
%   \caption{Seven Mode Planner Comparison.}
%   \label{fig:submodes3}
% \end{subfigure}
% \caption{State trajectories for the non-robust, unitary-consensus, and maximum-consensus approaches subject to a rotor failure induced at time $t=1s$ and a delayed IMM diagnosis of $+0.15s$.}
% \label{fig:modes}
% \end{figure*}

% % \newpage 
% \begin{figure*}[b!]
% \centering
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=1.0\linewidth]{CDC2023/Figures/3dtrajectory.png}
%   \caption{Visualization of the trajectories in 3D-space.}
%   \label{fig:sub1}
% \end{subfigure}%
% \begin{subfigure}{.5\textwidth}
%   \centering
%   \includegraphics[width=0.9\linewidth]{CDC2023/Figures/topview.png}
%   \caption{Top-view of the trajectories.}
%   \label{fig:sub2}
% \end{subfigure}
% \caption{Trajectory of the three methods: (1) non-robust, (2) unitary-consensus, and (3) maximum-consensus. It is observed that the maximum consensus algorithm is the only method capable of safely guiding the hexacopter to the goal state, even under a stochastic rotor failure.}
% \label{fig:trajectory}
% \end{figure*}
% \clearpage
% \subsection{Figures and Tables}

% Positioning Figures and Tables: Place figures and tables at the top and bottom of columns. Avoid placing them in the middle of columns. Large figures and tables may span across both columns. Figure captions should be below the figures; table heads should appear above the tables. Insert figures and tables after they are cited in the text.

% \begin{table}[h]
% \caption{An Example of a Table}
% \label{table_example}
% \begin{center}
% \begin{tabular}{|c||c|}
% \hline
% One & Two\\
% \hline
% Three & Four\\
% \hline
% \end{tabular}
% \end{center}
% \end{table}
%    \begin{figure}[thpb]
%       \centering
%       \framebox{\parbox{3in}{We suggest that you use a text box to insert a graphic (which is ideally a 300 dpi TIFF or EPS file, with all fonts embedded) because, in an document, this method is somewhat more stable than directly inserting a picture.
% }}
%       %\includegraphics[scale=1.0]{figurefile}
%       \caption{Inductance of oscillation winding on amorphous
%        magnetic core versus DC bias magnetic field}
%       \label{figurelabel}
%    \end{figure}

==> IROS2024/Bin/old_bib.tex <==
% \begin{thebibliography}{99}

% \bibitem{c1} G. O. Young, structure of industrial plastics ,.
% % \bibitem{c2} W.-K. Chen, Linear Networks and Systems (Book style).	Belmont, CA: Wadsworth, 1993, pp. 123Ð135.
% % \bibitem{c3} H. Poor, An Introduction to Signal Detection and Estimation.   New York: Springer-Verlag, 1985, ch. 4.
% % \bibitem{c4} B. Smith, ÒAn approach to graphs of linear forms (Unpublished work style),Ó unpublished.
% % \bibitem{c5} E. H. Miller, ÒA note on reflector arrays (Periodical styleÑAccepted for publication),Ó IEEE Trans. Antennas Propagat., to be publised.
% % \bibitem{c6} J. Wang, ÒFundamentals of erbium-doped fiber amplifiers arrays (Periodical styleÑSubmitted for publication),Ó IEEE J. Quantum Electron., submitted for publication.
% % \bibitem{c7} C. J. Kaufman, Rocky Mountain Research Lab., Boulder, CO, private communication, May 1995.
% % \bibitem{c8} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ÒElectron spectroscopy studies on magneto-optical media and plastic substrate interfaces(Translation Journals style),Ó IEEE Transl. J. Magn.Jpn., vol. 2, Aug. 1987, pp. 740Ð741 [Dig. 9th Annu. Conf. Magnetics Japan, 1982, p. 301].
% % \bibitem{c9} M. Young, The Techincal Writers Handbook.  Mill Valley, CA: University Science, 1989.
% % \bibitem{c10} J. U. Duncombe, ÒInfrared navigationÑPart I: An assessment of feasibility (Periodical style),Ó IEEE Trans. Electron Devices, vol. ED-11, pp. 34Ð39, Jan. 1959.
% % \bibitem{c11} S. Chen, B. Mulgrew, and P. M. Grant, ÒA clustering technique for digital communications channel equalization using radial basis function networks,Ó IEEE Trans. Neural Networks, vol. 4, pp. 570Ð578, July 1993.
% % \bibitem{c12} R. W. Lucky, ÒAutomatic equalization for digital communication,Ó Bell Syst. Tech. J., vol. 44, no. 4, pp. 547Ð588, Apr. 1965.
% % \bibitem{c13} S. P. Bingulac, ÒOn the compatibility of adaptive controllers (Published Conference Proceedings style),Ó in Proc. 4th Annu. Allerton Conf. Circuits and Systems Theory, New York, 1994, pp. 8Ð16.
% % \bibitem{c14} G. R. Faulhaber, ÒDesign of service systems with priority reservation,Ó in Conf. Rec. 1995 IEEE Int. Conf. Communications, pp. 3Ð8.
% % \bibitem{c15} W. D. Doyle, ÒMagnetization reversal in films with biaxial anisotropy,Ó in 1987 Proc. INTERMAG Conf., pp. 2.2-1Ð2.2-6.
% % \bibitem{c16} G. W. Juette and L. E. Zeffanella, ÒRadio noise currents n short sections on bundle conductors (Presented Conference Paper style),Ó presented at the IEEE Summer power Meeting, Dallas, TX, June 22Ð27, 1990, Paper 90 SM 690-0 PWRS.
% % \bibitem{c17} J. G. Kreifeldt, ÒAn analysis of surface-detected EMG as an amplitude-modulated noise,Ó presented at the 1989 Int. Conf. Medicine and Biological Engineering, Chicago, IL.
% % \bibitem{c18} J. Williams, ÒNarrow-band analyzer (Thesis or Dissertation style),Ó Ph.D. dissertation, Dept. Elect. Eng., Harvard Univ., Cambridge, MA, 1993. 
% % \bibitem{c19} N. Kawasaki, ÒParametric study of thermal and chemical nonequilibrium nozzle flow,Ó M.S. thesis, Dept. Electron. Eng., Osaka Univ., Osaka, Japan, 1993.
% % \bibitem{c20} J. P. Wilkinson, ÒNonlinear resonant circuit devices (Patent style),Ó U.S. Patent 3 624 12, July 16, 1990. 


% \end{thebibliography}



==> IROS2024/Inputs/acronyms.tex <==
\newacronym{cbf}{CBF}{Control Barrier Function}
\newacronym{mdp}{MDP}{Markov Decision Process}
\newacronym{sos}{SoS}{Sum-of-Squares}
\newacronym{sdp}{SDP}{Semi-definite Programming}
\newacronym{bnn}{BNN}{Bayesian Neural Network}
\newacronym{stl}{STL}{Signal Temporal Logic}
\newacronym{hjr}{HJR}{Hamilton-Jacobi Reachability}
\newacronym{psd}{PSD}{Positive Semi-Definite}
\newacronym{smt}{SMT}{Satisfiability Modulo Theory}
\newacronym{milp}{MILP}{Mixed-Integer Linear Programming}
\newacronym{lbp}{LBP}{Linear Bound Propagation}
\newacronym{ibp}{IBP}{Interval Bound Propagation}
\newacronym{nn}{NN}{Neural Network}
\newacronym{nbf}{NBF}{Neural Barrier Function}

==> IROS2024/Sections/2_Preliminaries.tex <==
\section{Preliminaries}

\subsection{Filter}
\ZL{Talk about sojourn time for mode detection}


\subsection{Model Predictive Control}




